Infinite-order diagrammatic summation approach to explicitly correlated congruent transformed Hamiltonian

A resolution of identity approach to explicitly correlated congruent transformed Hamiltonian (CTH) is presented. One of the principle challenges associated with the congruent transformation of the many-electron Hamiltonian is the generation of three, four, five, and six particle operators. Successful application of the congruent transformation requires efficient implementation of the many-particle operators. In this work, we present the resolution of identity congruent transformed Hamiltonian (RI-CTH) method to handle many-particle operators. The resolution of identity was used to project the explicitly correlated operator in a N-particle finite basis to avoid explicit computation of the many-particle operators. Single-particle states were obtained by performing Hartee-Fock calculations, which were then used for construction of many-particle states. The limitation of the finite nature of the resolution of identity was addressed by developing partial infinite order (PIOS) diagrammatic summation technique. In the PIOS method, the matrix elements of the projected congruent transformed Hamiltonian was expressed in terms of diagrammatic notation and a subset of diagrams were summed up to infinite order. The RI-CTH and RI-CTH-PIOS methods were applied to isoelectronic series of 10-electron systems (Ne,HF,H2O,NH3,CH4) and results were compared with CISD and CCSD(T) calculations. One of the key results from this work is that for identical basis set, the RI-CTH-PIOS energies are lower than CISD and CCSD(T) values.

==> section_dir/sec_acknowledgements.tex <==
We gratefully acknowledge the support from Syracuse
University for this work.

==> section_dir/sec_ref.tex <==
\begin{itemize}
  \item Author: Bubin, Adamowicz findings: Presented an algorithm for the variational calculation 
        of atomic D states employing n-electron explicitly correlated Gaussians. This method was 
        tested on the two lowest D states of lithium and beryllium atoms. The lowest D state of Li 
        presented is lower than the best preiously reported result.\cite{sharkey2011algorithm}

  \item Author: Bubin, Adamowicz findings: The nine lowest members of the $^{2}P^{0}$ Rydberg series 
        of the Lithium atom are studied using accurate quantum-mechanical nonrelativistic variational 
        methods. The wave functions of the staes are expanded in terms of all-electron explicitly 
        correlated energy levels. The variational parameters of the Gaussinas are variationally 
        optimized.\cite{bubin2012explicitly}
  
  \item Author: Adamowicz findings: Explicitly correlated, n-electron, one-center s Gaussian (ECG) 
        functions are combined with s ECGs through pre-exponential $r_{ij}^{2}$ multipliers. The pre-
        exponentially $r_{ij}^{2}$-dependent ECGs are included in the basis to better describe the 
        interelectron correlation and the interelectron cusps. The was tested for the ground state of 
        the beryllium atom.\cite{sharkey2011exponentially}

  \item Author: Lane findings: Studied the equilibrium geometry of water and water dimer using coupled 
        cluster theory. The geometries were optimized using coupled cluster methods using singles, 
        doubles, triples, and quadruple excitations CCSDTQ. Explicitly correlated coupled cluster 
        singles, doubles and perturbative triples CCSD(T)-F12b was also used.\cite{lane2012ccsdtq}
        

  \item Author: Manby findings: Treats electron correlation where a correlation factor is optimized 
        using Hylleraas variational perturbation theory. Tested the method on Helium system with a 
        result of -2.9035.\cite{manby1999real}

  \item Author: Tew, Klopper, Manby findings: The weak othrogonality functional and the resolution of 
        identity are examined using MP2-GTG. Proposes a new weak orthogonality funcitonal where the 
        explicitly correlated pair functions are almost orthogonal to the occupied orbitals by 
        construction.\cite{tew2007weak} 

  \item Author: Manby, Werner, Adler, May findings: Used the MP2-R12/2*A(loc) and LMP2-R12/2*A(loc) 
        methods are modified to use a short-rang correlation factor expanded as a fixed linear 
        combination of Gaussian geminals. The short-range correlation factor leads to improved 
        convergence of RI and eliminates problems with long-range errors in density fitting caused 
        by the linear $r_{12}$ factor. This work is applied to 21 small molecules in which correlation 
        energy is calculated.\cite{manby2006explicitly}

  \item Author: Ten-no, Manby findings: Used explicitly correlated second order MBPT. It is shown that 
        the convergence of R12-type explicitly correlated electronic structure theories can be improved 
        by rearranging the three-electron integrals before using a resolution of the identity to decompose 
        them into expressions involving only two-electron integrals.\cite{ten2003density}

  \item Author: Valeev, Hirata findings: CCSD or CCSDT with noniterative, perturbation corrections for 
        higher order excitations has been extended to include the basis functions that explicitly 
        depend on intereclectronic distances in the wavefunction expansions.\cite{shiozaki2009explicitly}

  \item Author: Valeev, Hirata findings: CCSD-R12 was implemented based on the nontruncated formalisms 
        in which every diagrammatic term that arises from the modified ansatz is evaluated either 
        analytically or by using RI insertion with the complementary auxiliary basis set. Correlation 
        energies and percent correlation are reported for the systems Ne, H$_{2}$O, and F$_{2}$.\cite{shiozaki2008explicitly}

  \item Author: Valeev findings: Extended the perturbative explicitly correlated CCSD method to account 
        for the effect of connected three-electron correlations.\cite{valeev2008simple}

  \item Author: Valeev findings: Presents a general MP2-R12 method in which each electron pair uses a 
        st of perturbative explicitly correlated contraced GTGs with fixed exponents, whose coefficients 
        are optimized linearly. In this method, only two-electron integrals are needed, the only approximations 
        are the RI and Brillouin condition, only linear parameters are optimized, and an arbitrary 
        number of perturbative explicitly correlated non-contracted GTGs can appear.\cite{valeev2006combining}

  \item Author: Valeev findings: Expanded the orthogonal complement to the span of orbital basis set (OBS). The 
        new formulation presented is called complementary auxiliary basis set (CABS) MP2-R12 method. RI is used 
        in this method in approximating many-electron matrix elements. Studied whether there is a better approach 
        than direct insertion of the RI in the three-electron integrals.\cite{valeev2004improving}

  \item Author: Klopper, Samson findings: Uses RI in explicitly correlated MP2-R12 method to treat 
        the three- and four-electron integrals in terms of the one-electron basis. In this work, an 
        auxiliary basis set is used to represent the RI instead of a singls basis.\cite{klopper2002explicitly} 

  \item Author: Rassolov findings: The cusp condition is a consequence of the Coulomb singularity in the 
        potential and provides a specific relation betwee the wavefunction and its first derivative at the point 
        of coalescence.\cite{rassolov1996behavior}

  \item Author: Alavi, Booth findings: Developed a new FCI-QMC method and is tested on a number of many-
        electron systems.\cite{booth2009fermion}

  \item Author: Bartlet findings: Diagrammatic perturbation theory. Goldstone diagrams.\cite{shavitt2009many}

  \item Author: Kohn, Tew findings: The equations of explicitly correlated coupled cluster singles and 
        doubles (CCSD-F12) were analyzed\cite{kohn2010explicitly} 

  \item Author: Kohn, Hattig findings: Propsed a novel explicitly correlated coupled-cluster singles 
        and doubles CCSD(F12*) method which has computational costs close to that of CCSD, but retains 
        of CCSD-F12.\cite{hattig2010communications}

  \item Author: Kohn findings: Incorporates explicit electron correlation into connected triple 
        excitations using coupled-cluster.\cite{kohn2009explicitly}

  \item Author: Hirata, Valeev findings: Implemented explicitly correlated coupled-cluster (CC-R12 or CC-F12) 
        methods with up to triple and quadruple excitations (CCSDT-R12 and CCSDTQ-R12). Reports results for 
        water and compares with CBS extrapolations and experimental and theoretical studies. Reports the 
        energy for water as -76.437 +/- 0.003 using CCSDTQ-R12 method.\cite{shiozaki2009higher}

  \item Author Scuseria findings: Introduces a method that uses a wavefunction that is a Jastrow function 
        multiplied by the sum of Slater determinants in QMC methods. VMC and DMC methods using single 
        determinant and multi-Slater determinant Jastrow functions are used to compute ground state 
        energy for water. The work reports the energy of water to be -76.4306(9) for VMC-MSDJ, and -76.4368(4) 
        for DMC-MSDJ.\cite{clark2011computing}

  \item Author So Hirata findings: Presents second order MP2-R12 or F12 method in which the basis functions 
        depend explicitly on electron-electron distances. Many-electron integrals over Gaussian-type 
        functions involving Slater-type geminals are evaluated using RI approximation with a complementary 
        auxiliary basis set.\cite{shiozaki2010communications} 

  \item Author Drake findings: Discusses variational techniques which improve the accuracy of the eigenvalues 
        for helium by several magnitudes.\cite{drake1989new}

  \item Author Wagner findings: Performs high-accuracy DMC calculations with explicit electron-electron 
        correlation on MnO and TiO\cite{wagner2003quantum} 

  \item Author Head-Gordon findings: Proposes a perturbative version of their coupled-cluster models 
        for the total energy based on a local, active-space treatment of the valence problem built 
        of correlated electron pairs.\cite{parkhill2011formulation} 

  \item Author Head-Gordon findings: Investigates a metric that involves only local or semilocal 
        operators and reduces the two-electron Coulomb operator into sums over one-electron terms. 
        They introduce the expansion of the resolution of the identity MP2 (RI-MP2).\cite{lambrecht2011kinetic}

\end{itemize}


==> section_dir/table2.tex <==
Since the challenge of this paper was to extend the CTH method to systems 
with many electrons, the 10 electron systems, $\mathrm{Ne}$, $\mathrm{HF}$, 
$\mathrm{H_{2}O}$, $\mathrm{NH_{3}}$, and $\mathrm{CH_{4}}$ were tested. \autoref{tab:ten_elec} 
shows the results of these calculations using the 6-31$\mathrm{G}^{\star\star}$ basis set.  
   %%  \begin{table}[ht]
   %%  %\textcolor{BlueViolet}{\noindent\hrulefill}
   %%    \begin{center}
   %%     \caption{\textbf{Test for H$_{2}$O calculation. Energies [Hartrees] are with respect 
   %%                      to the Hartree-Fock energy}}
   %%     \label{tab:water_results}
   %%      \begin{tabular}{ l l c }  
   %%       %\rowcolor{lightgray} $\textbf{Method/Basis Set}$     &  $\textbf{Energy[Hartrees]}$ \\
   %%          $\textbf{Method/Basis Set}$     &  $\textbf{Energy[Hartrees]}$   & $\textbf{References}$ \\
   %%          $\mathrm{\textrm{RI\text{-}CTH}/6\text{-}31G^{\star}}$          &  -76.165385  & $\textrm{This work}$  \\ 
   %%          $\mathrm{\textrm{RI\text{-}CTH\text{-}PIOS}/6\text{-}31G^{\star}}$     &  -76.323653  & $\textrm{This work}$  \\ 
   %%          $\mathrm{\textrm{CISD}/6\text{-}31G^{\star}}$            &  -76.198206  & \cite{johnson2010computational}\\  
   %%          $\mathrm{\textrm{CCSD(T)}/6\text{-}31G^{\star}}$         &  -76.205841  & \cite{johnson2010computational}\\  
   %%      \end{tabular}
   %%    \end{center}  
   %%  %\textcolor{BlueViolet}{\noindent\hrulefill}
   %%  \end{table}   
From \autoref{tab:ten_elec} it is shown that the CISD energy is lower than the 
RI-CTH energy. However, the RI-CTH-PIOS energy is lower than the CISD energy. Thus, 
the addition of the PIOS correction on the RI-CTH energy brings the energy lower than 
the CISD energy. This illustrates very well the importance of the infinite summation 
of the certain class of diagrams becuase the PIOS correction includes terms that are 
not present in the CISD energy. 
Furthermore, the RI-CTH-PIOS energy for $\mathrm{H_{2}O}$ with the 6-31$\mathrm{G}^{\star\star}$ 
basis set was compared to CISD and CCSD(T) results using much larger cc-pV(T+d)Z basis set. 
The results of this comparison along with other methods are displayed in \autoref{tab:h2o_compare}.  
\begin{table}[ht]
%\textcolor{BlueViolet}{\noindent\hrulefill}
  \begin{center}
   %\caption{\textbf{RI-CTH-PIOS comparison with large basis sets (Alavi geometry rOH=0.975512, $\theta$=110.565$^{\circ}$)}}
   \caption{\textbf{RI-CTH-PIOS comparison with large basis sets }}
   \label{tab:h2o_compare}
    \begin{tabular}{ l l c }  
    \hline
     %\rowcolor{lightgray} $\textbf{Method/Basis Set}$   &  $\textbf{Energy[Hartrees]}$ \\
        $\textbf{Method/Basis Set}$                          &  $\textbf{Energy[Hartrees]}$       & $\textbf{References}$  \\ \hline
        $\mathrm{\textrm{RI\text{-}CTH}/6\text{-}31G^{\star}}$             &  -76.165385          & $\textrm{This work}$  \\ 
        $\mathrm{\textrm{CISD}/6\text{-}31G^{\star}}$                      &  -76.198206          & \cite{johnson2010computational} \\  
        $\mathrm{\textrm{CCSD(T)}/6\text{-}31G^{\star}}$                   &  -76.205841          & \cite{johnson2010computational} \\  
        $\mathrm{\textrm{FCI\text{-}QMC/cc\text{-}pVDZ}}$                  &  -76.24186           & \cite{booth2009fermion} \\
        $\mathrm{\textrm{CCSD(T)}/jun\text{-}cc\text{-}pVDZ}$              &  -76.25755996        & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{CCSDT(Q)}/jun\text{-}cc\text{-}pVDZ}$             &  -76.25829015        & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{FCI\text{-}QMC/cc\text{-}pCVDZ}}$                 &  -76.28091(3)        & \cite{booth2009fermion} \\
        $\mathrm{\textrm{RI\text{-}CTH\text{-}PIOS}/6\text{-}31G^{\star}}$ &  -76.311230          & $\textrm{This work}$  \\ 
        $\mathrm{\textrm{CISD}/cc\text{-}pV(T+d)Z}$                        &  -76.313875          & \cite{johnson2010computational} \\
        $\mathrm{\textrm{CCSD(T)}/cc\text{-}pV(T+d)Z}$                     &  -76.324556          & \cite{johnson2010computational} \\
        $\mathrm{\textrm{CCSD(T)}/may\text{-}cc\text{-}pVTZ}$              &  -76.33700993        & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{CCSDT(Q)}/may\text{-}cc\text{-}pVTZ}$             &  -76.33746459        & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{VMC\text{-}singleDet}}$                           &  -76.3938(4)         & \cite{clark2011computing} \\
        $\mathrm{\textrm{DMC\text{-}singleDet}}$                           &  -76.4236(2)         & \cite{clark2011computing} \\
        $\mathrm{\textrm{VMC\text{-}MSDJ}}$                                &  -76.4306(9)         & \cite{clark2011computing} \\
        $\mathrm{\textrm{CCSD(T)}/aug\text{-}cc\text{-}pwCV5Z}$            &  -76.43229082        & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{CCSD(T)\text{-}F12}/aug\text{-}cc\text{-}pCVQZ\text{-}F12}$   &  -76.43661713 & \cite{lane2012ccsdtq} \\
        $\mathrm{\textrm{DMC\text{-}MSDJ}}$                                &  -76.4368(4)         & \cite{clark2011computing} \\
        $\mathrm{\textrm{CCSDTQ\text{-}R12/aug\text{-}cc\text{-}pCVQZ}}$   &  -76.437$\pm$0.003   & \cite{shiozaki2009higher} \\
        $\mathrm{\textrm{CEEIS\text{-}FCI+CBS}}$                           &  -76.4390$\pm$0.0004 & \cite{bytautas2006correlation} \\
      \hline
    \end{tabular}
  \end{center}  
%\textcolor{BlueViolet}{\noindent\hrulefill}
\end{table}   
The CISD and CCSD(T) results with the much larger basis are comparable in terms of energy 
with the RI-CTH-PIOS energy with only the 6-31$\mathrm{G}^{\star\star}$ basis. The RI-CTH-PIOS energy is 
actually lower in energy than the CISD energy with the much larger basis. The RI-CTH-PIOS method 
is compared to other methods as well.

